Hydrogen Masers. I: Theory and Prospects

The discovery of the first naturally occurring high gain hydrogen recombination line (HRL) maser, in the millimeter and submillimeter spectrum of the emission line star MWC349, requires an expansion of current paradigms about HRLs. In this paper we re-examine in general the physics of non-LTE populations in recombining hydrogen and specify the conditions necessary for high-gain masing and lasing in HRLs. Saturation of masing recombination lines is a critical consideration. We draw attention to another non-LTE phenomenon active in hydrogen: the overcooling} of populations. Observationally the HRL overcooling might manifest itself as an anomalously weak emission recombination line, or as a ``dasar,'' that is, an anomalously strong absorption line. We briefly discuss the prospects of detecting hydrogen masers, lasers and dasars in several classes of galactic and extragalactic objects, including compact HII regions, Be or Wolf-Rayet stars, and AGNs.

==> table.tex <==
\magnification=\magstep0
\vsize=23.5truecm
\hsize=16.0truecm
\centerline{\vbox{
\tabskip=0pt \offinterlineskip
\def\tablerule{\noalign{\vskip2pt\hrule\vskip3pt}}
\def\skip{\noalign{\vskip4pt}}
\halign to \hsize {\tabskip=1em plus2em
\hfil#&\hfil#\hfil&\hfil#\hfil&\hfil#\hfil&\hfil#\hfil&$\quad#$&
\hfil#\hfil&\hfil#\hfil&\hfil#\hfil&\hfil#\hfil\tabskip=0pt\cr\tablerule
\omit&\multispan4\hfil$T_e=5\,10^3\;$K\hfil&&
\multispan4\hfil$T_e=10^4\;$K\hfil\cr\noalign{\vskip2pt}
\omit&\multispan4\hrulefill&&\multispan4\hrulefill\cr\noalign{\vskip4pt}
\omit&\multispan2\hfil$\alpha$-lines\hfil&\multispan2\hfil$\beta$-lines\hfil
&&\multispan2\hfil$\alpha$-lines\hfil&\multispan2\hfil$\beta$-lines\hfil
\cr\noalign{\vskip2pt}
&\multispan4\hrulefill&&\multispan4\hrulefill\cr\noalign{\vskip4pt}
n\hfil
&$k_{net}^{max},$&$N_e^{max},$
&$k_{net}^{max},$&$N_e^{max},$&
&$k_{net}^{max},$&$N_e^{max},$
&$k_{net}^{max},$&$N_e^{max},$
\cr\noalign{\vskip2pt}
%
\omit
&cm$^{-1}$&cm$^{-3}$
&cm$^{-1}$&cm$^{-3}$&
&cm$^{-1}$&cm$^{-3}$
&cm$^{-1}$&cm$^{-3}$
\cr\noalign{\vskip2pt}
&\multispan4\hrulefill&&\multispan4\hrulefill\cr\noalign{\vskip4pt}
%
$  5$&$-6.9\;10^{-8}$&$8.9\;10^{11}$&$-5.1\;10^{-9}$&$6.3\;10^{11}$&
&$-6.1\;10^{-9}$&$8.9\;10^{11}$&$-4.8\;10^{-10}$&$6.3\;10^{11}$\cr\skip
$ 10$&$-8.8\;10^{-11}$&$1.3\;10^{10}$&$-8.8\;10^{-12}$&$1.0\;10^{10}$&
&$-2.1\;10^{-11}$&$1.8\;10^{10}$&$-1.8\;10^{-12}$&$1.3\;10^{10}$\cr\skip
$ 15$&$-2.4\;10^{-12}$&$1.1\;10^9$&$-2.6\;10^{-13}$&$1.0\;10^9$&
&$-6.2\;10^{-13}$&$1.6\;10^9$&$-7.1\;10^{-14}$&$1.4\;10^9$\cr\skip
$ 20$&$-2.5\;10^{-13}$&$2.2\;10^8$&$-2.9\;10^{-14}$&$2.0\;10^8$&
&$-8.1\;10^{-14}$&$3.5\;10^8$&$-9.0\;10^{-15}$&$3.2\;10^8$\cr\skip
$ 25$&$-4.8\;10^{-14}$&$7.1\;10^7$&$-5.6\;10^{-15}$&$6.3\;10^7$&
&$-1.5\;10^{-14}$&$1.1\;10^8$&$-1.6\;10^{-15}$&$8.9\;10^7$\cr\skip
$ 30$&$-1.2\;10^{-14}$&$2.5\;10^7$&$-1.4\;10^{-15}$&$2.2\;10^7$&
&$-3.5\;10^{-15}$&$4.0\;10^7$&$-3.4\;10^{-16}$&$2.8\;10^7$\cr\skip
$ 35$&$-3.7\;10^{-15}$&$1.1\;10^7$&$-4.1\;10^{-16}$&$1.0\;10^7$&
&$-9.6\;10^{-16}$&$1.4\;10^7$&$-8.4\;10^{-17}$&$1.1\;10^7$\cr\skip
$ 40$&$-1.3\;10^{-15}$&$5.6\;10^6$&$-1.4\;10^{-16}$&$4.5\;10^6$&
&$-2.9\;10^{-16}$&$6.3\;10^6$&$-2.3\;10^{-17}$&$4.0\;10^6$\cr\skip
$ 45$&$-4.9\;10^{-16}$&$2.5\;10^6$&$-4.9\;10^{-17}$&$2.0\;10^6$&
&$-9.2\;10^{-17}$&$2.5\;10^6$&$-6.5\;10^{-18}$&$1.6\;10^6$\cr\skip
$ 50$&$-2.0\;10^{-16}$&$1.4\;10^6$&$-1.8\;10^{-17}$&$1.0\;10^6$&
&$-3.1\;10^{-17}$&$1.3\;10^6$&$-2.0\;10^{-18}$&$7.1\;10^5$\cr\skip
$ 55$&$-8.4\;10^{-17}$&$7.1\;10^5$&$-7.2\;10^{-18}$&$5.0\;10^5$&
&$-1.1\;10^{-17}$&$5.6\;10^5$&$-6.7\;10^{-19}$&$3.2\;10^5$\cr\skip
$ 60$&$-3.7\;10^{-17}$&$4.0\;10^5$&$-2.9\;10^{-18}$&$2.5\;10^5$&
&$-4.2\;10^{-18}$&$2.8\;10^5$&$-2.4\;10^{-19}$&$1.4\;10^5$\cr\skip
$ 65$&$-1.7\;10^{-17}$&$2.2\;10^5$&$-1.2\;10^{-18}$&$1.4\;10^5$&
&$-1.7\;10^{-18}$&$1.4\;10^5$&$-8.9\;10^{-20}$&$7.1\;10^4$\cr\skip
$ 70$&$-7.8\;10^{-18}$&$1.3\;10^5$&$-5.4\;10^{-19}$&$7.9\;10^4$&
&$-7.0\;10^{-19}$&$7.1\;10^4$&$-3.5\;10^{-20}$&$3.5\;10^4$\cr\skip
$ 75$&$-3.7\;10^{-18}$&$7.1\;10^4$&$-2.4\;10^{-19}$&$4.5\;10^4$&
&$-3.1\;10^{-19}$&$4.0\;10^4$&$-1.5\;10^{-20}$&$2.0\;10^4$\cr\skip
$ 80$&$-1.8\;10^{-18}$&$4.5\;10^4$&$-1.1\;10^{-19}$&$2.5\;10^4$&
&$-1.4\;10^{-19}$&$2.2\;10^4$&$-6.3\;10^{-21}$&$1.1\;10^4$\cr\skip
$ 85$&$-9.3\;10^{-19}$&$2.8\;10^4$&$-5.5\;10^{-20}$&$1.4\;10^4$&
&$-6.5\;10^{-20}$&$1.3\;10^4$&$-2.9\;10^{-21}$&$6.3\;10^3$\cr\skip
$ 90$&$-4.8\;10^{-19}$&$1.6\;10^4$&$-2.7\;10^{-20}$&$8.9\;10^3$&
&$-3.2\;10^{-20}$&$7.9\;10^3$&$-1.4\;10^{-21}$&$3.5\;10^3$\cr\skip
$ 95$&$-2.5\;10^{-19}$&$1.0\;10^4$&$-1.4\;10^{-20}$&$5.6\;10^3$&
&$-1.6\;10^{-20}$&$4.5\;10^3$&$-6.7\;10^{-22}$&$2.0\;10^3$\cr\skip
$100$&$-1.4\,10^{-19}$&$6.3\,10^3$&$-7.3\,10^{-21}$&$3.2\,10^3$&
&$-8.3\,10^{-21}$&$2.8\,10^3$&$-3.4\,10^{-22}$&$1.3\,10^3$\cr\tablerule
}}}
\end


